Decentralised Active Perception in Continuous Action Spaces for the Coordinated Escort Problem

We consider the coordinated escort problem, where a decentralised team of supporting robots implicitly assist the mission of higher-value principal robots. The defining challenge is how to evaluate the effect of supporting robots' actions on the principal robots' mission. To capture this effect, we define two novel auxiliary reward functions for supporting robots called satisfaction improvement and satisfaction entropy, which computes the improvement in probability of mission success, or the uncertainty thereof. Given these reward functions, we coordinate the entire team of principal and supporting robots using decentralised cross entropy method (Dec-CEM), a new extension of CEM to multi-agent systems based on the product distribution approximation. In a simulated object avoidance scenario, our planning framework demonstrates up to two-fold improvement in task satisfaction against conventional decoupled information gathering.The significance of our results is to introduce a new family of algorithmic problems that will enable important new practical applications of heterogeneous multi-robot systems.

==> atomic_comments.tex <==
(1) Speak more broadly about the applicability of DecCEM, its computational complexity and applications in other areas. 


(3) Problem formulation. 
    - Says by stacking all states together, transition dyanmics, and observation function we can use any standard stochastic motion planning problem. Want as a baseline
    - Why use CEM? Why not iLGQ? In reach-avoid this will work well, so if motivating use by temporal logic, why don't experiments reflect this?
    - Mention why we chose the PA speed as we did.
    - 
(2) Figure 2...
    - Connect to equation 7

(4) Figure 3...
    - Reviewers believe it doesn't make sense. Why doesn't performance improve as there are more agents?

(5) Figure 4...
    - Blind strategy needs more explanation
    - Exemplary figure that supports the main evaluations.
    - "Interesting that the beliefs of some obstacles are not increased, but decreased over time"

(6) Experiments
    - Weak. 
    - Comparisons between SI/SE are not well-explained.
    - Want proper statistical analysis (e.g. standard errors etc).
    - Want more. 
    - If not more, explain the difficulties of this problem setup.

(7) DecCEM
    - Want either a better discussion on the broader applicability of DecCEM or WHY we limited to the coordinated escorting problem.
    - What is the computational complexity -- please include
    - Why decentralised if all information is shared across robots?
    - Prove it will eventually converge
    - Why wouldn't async comms break this? (we only show that everyone communicates at a single step?)

(8) Equation 6: 
    - Is there a typo in eq 6 as p(phi | x, y) <= p(phi|x)?

Typos/grammar:	
    - “The SE approaches demonstrates” (pg 2, paragraph 2)
    - “when a principal agent planning over the prior alone.” (pg 2, paragraph 3)
    - References 11, 20
    

